A Good Talk Does not Look Like a Summary, It Teaches You! Measuring Takeaways from Paper-to-Video Talks

Automatically generated videos from scientific papers are increasingly used for education and research dissemination. However, existing evaluation metrics mainly measure visual quality or whether key points from the paper appear in the video without assessing whether the video actually helps viewers understand the ideas. We introduce EffectivePresentationScorer, a framework for evaluating the instructional quality of scientific presentation videos. It checks whether a video explains the main ideas clearly, introduces needed background concepts, and connects technical details to the main contribution of the paper. When we apply EffectivePresentationScorer to the existing paper-to-video generation systems, we find that generated videos mention the correct topics and follow the structure of the paper but fail to explain prerequisite concepts or clarify why the method works. These failures are often ignored by existing video evaluation metrics, which focus on content presence rather than explanatory quality.

==> acl_lualatex.tex <==
% % This file compiles with both LuaLaTeX and XeLaTeX
% \documentclass[11pt]{article}

% % Change "review" to "final" to generate the final (sometimes called camera-ready) version.
% % Change to "preprint" to generate a non-anonymous version with page numbers.
% \usepackage[review]{acl}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
%  \usepackage{microtype}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% % These font selection commands work with
% % LuaLaTeX and XeLaTeX, but not pdfLaTeX.
% \usepackage[english,bidi=default]{babel} % English as the main language.
% \babelfont{rm}{TeXGyreTermesX} % similar to Times
% %%% include whatever languages you need below this line
% \babelprovide[import]{hindi}
% \babelfont[*devanagari]{rm}{Lohit Devanagari}
% \babelprovide[import]{arabic}
% \babelfont[*arabic]{rm}{Noto Sans Arabic}


% %\usepackage{polyglossia}
% %\setdefaultlanguage{english}
% %\setotherlanguages{arabic,russian,thai,hindi,kannada}

% %%%%%


% \title{LuaLaTeX and XeLaTeX Template for *ACL Style Files}

% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row'' of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% \author{First Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\\And
%   Second Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\}

% \begin{document}

% \maketitle
% \begin{abstract}
% This document provides an example showing how
% to use the *ACL style files with either
% LuaLaTeX or XeLaTeX.
% \end{abstract}


% \section{Introduction}

% Please see the general instructions
% in the file \verb|acl_latex.tex|.

% Here are some examples of text in various languages.

% Hindi: \foreignlanguage{hindi}{मानव अधिकारों की सार्वभौम घोषणा}

% Arabic: \foreignlanguage{arabic}{الإعلان العالمي لحقوق الإنسان}

% Here is an example citation:
% \citet{Gusfield:97} argues that...


% % Entries for the entire Anthology, followed by custom entries
% \bibliography{custom}

% \appendix

% \section{Example Appendix}
% \label{sec:appendix}

% This is an appendix.

% \end{document}

